Clustering Techniques for Stable Linear Dynamical Systems with applications to Hard Disk Drives

In Robust Control and Data Driven Robust Control design methodologies, multiple plant transfer functions or a family of transfer functions are considered and a common controller is designed such that all the plants that fall into this family are stabilized. Though the plants are stabilized, the controller might be sub-optimal for each of the plants when the variations in the plants are large. This paper presents a way of clustering stable linear dynamical systems for the design of robust controllers within each of the clusters such that the controllers are optimal for each of the clusters. First a k-medoids algorithm for hard clustering will be presented for stable Linear Time Invariant (LTI) systems and then a Gaussian Mixture Models (GMM) clustering for a special class of LTI systems, common for Hard Disk Drive plants, will be presented.

==> references.tex <==
\begin{thebibliography}{00}  % you can also add the bibliography by hand

%\bibitem[Kasavajhala(2011)]{Ka:11}
%V. Kasavajhala.
%\newblock Sold state drive vs. hard disk drive
%price and performance study
%\newblock \emph{Proc. Dell Tech. White Paper},  2011.

%\bibitem[Khargonekar et~al.(1991) Khargonekar and Rotea]{KhRo:91}
%P.P. Khargonekar and M.A. Rotea.
%newblock Mixed H2/H infinity
%control: A convex optimization approach.
%\newblock \emph{IEEE
%Transactions on Automatic Control}, volume~36(7), pages
%  824--837, 1991.
  
%\bibitem[Hast et~al (2013) Hast, Astrom,  Bernhardsson and Boyd]{HaAsBeBo:13}
%M.K. Hast, K. J. Astrom, B. Bernhardsson and S. Boyd
%\newblock PID design by convex-concave optimization, 
%\newblock \emph{European Control Conference}, pages 4460--4465, 2013.

%\bibitem[Zhou (1998)]{Zh:98}
%K. Zhou, 
%\newblock Essentials of Robust Control, Prentice
%Hall, New Jersey, 1998.

%\bibitem[Saeki (2014)]{Sa:14}
%M. Saeki, 
%\newblock Data-driven loop-shaping design
%of PID controllers for stable plants,
%\newblock \emph{International
%Journal of Adaptive Control and Signal Processing}, volume~28(12), pages 1325-1340, 2014.


\bibitem{Ba:17}
O. Bagherieh,
\newblock Estimation, identification and
data-driven control design for hard disk drives,
\newblock \emph{PhD thesis, University of California, Berkeley}, 2017. https://escholarship.org/uc/item/0998n097

\bibitem{Ni:22}
N.P.S.Prakash and R. Horowitz
\newblock Data-Driven Robust Feedback Control Design for Multi-Actuator hard Disk Drives
\newblock \emph{Modeling Estimation and Controls Conference}, 2022.

\bibitem{At:20}
T. Atsumi and S. Yabui
\newblock Quadruple-Stage Actuator System for Magnetic-Head Positioning System in HDDs 
\newblock \emph{The IEEE Transactions on Industrial
Electronics}, volume~67(11), pages 9184-9194, 2020.

\bibitem{Eg:17}
T. Eguchi, Y. Asai, K. Ichikawa, and M. Takada \newblock Airborne and Structure-Borne Transmission of High Frequency Fan Vibration in a Storage Box \newblock \emph{Proceedings of the ASME 2017 Conference on Information Storage and Processing
Systems}, paper No. 5406, 2017.

\bibitem{GaKaLo:10}
G. Galdos, A. Karimi and R. Longchamp
\newblock Hinfinity
controller design for spectral mimo models by convex
optimization.
\newblock \emph{Journal of Process Control}, volume~20(10), pages 1175--1182, 2010.

\bibitem{KaKa:17}
A. Karimi and C. Kammer
\newblock A data driven approach to robust
control of multivariable systems by convex optimization”.
\newblock \emph{Automatica}, 2017.

\bibitem{KaNiZh:16}
A. Karimi, A. Nicoletti and Y. Zhu
\newblock Robust hinfinity
controller design using frequency domain data via
convex optimization.
\newblock \emph{International Journal of Robust and
Non Linear Control}, volume~20(10), 2016.

%\bibitem[Bazanella et~al.(2011) Bazanella, Campestrini, and Eckhard]{BaCaEc:11}
%A.S. Bazanella, L. Campestrini, and D. Eckhard
%\newblock Data-driven controller design: the h2 approach.
%\newblock \emph{Springer
%Science and Business Media}, 2011.

%\bibitem[Boyd et~al (2016) Boyd, Hast and Astrom]{BoHaAs:16}
%S. Boyd, M. Hast and K.J. Astrom ,
%\newblock MIMO
%PID tuning via iterated LMI restriction
%\newblock \emph{ International
%Journal of Robust and Nonlinear Control}, volume~26(8) pages 1718--1731, 2016.

\bibitem{ShHo:20}
P. Shah and R. Horowitz, 
\newblock Data Driven Feedforward Control Design and Input Shaping Techniques for Multi Actuator Drives,
\newblock \emph{ASME 2020 Conference on Dynamics Systems and Control}, 2020.

\bibitem{ShChHo:20}
P. Shah, Z.Chen and R. Horowitz,
\newblock Application of MIMO Data Driven Feedback Control Design to Dual Stage Hard Disk Drives
\newblock \emph{ASME 2020 Conference on Dynamics Systems and Control}, 2020.


\bibitem{ChShHo:20}
Z. Chen, P. Shah and R. Horowitz,
\newblock Head-Positioning Control in Triple-Stage-Actuator Hard Disk Drives Using Mixed  Synthesis Methodologies
\newblock \emph{ASME 2020 Conference on Dynamics Systems and Control}, 2020.

\bibitem{ShHo:19}
P. Shah and R. Horowitz
\newblock Active Vibration Rejection in Multi Actuator Drives – Data Driven Approach 
\newblock \emph{ASME Conference on Dynamics Systems and Control} , 2019.

\bibitem{BaShHo:18}
O. Bagherieh, P. Shah and R. Horowitz,
\newblock Application of Mixed  Data Driven Control Design to Dual Stage Hard Disk Drives 
\newblock \emph{ASME Conference on Dynamics Systems and Control}, 2018.
 
 \bibitem{ShHo:21}
 P. Shah and R. Horowitz 
 \newblock Data Driven Feedforward Control Design and Input Shaping Techniques for Multi Actuator Drives. 
 \newblock \emph{ASME 2021 Letters in Dynamics Systems and Control}, 2021.
 
 \bibitem{PrChHo:22}
 N.P.S Prakash, Z. Chen and R. Horowitz. 
 \newblock Data-Driven Strictly Positive Real System Identification with prior
System Knowledge
\newblock \emph{American Controls Conference}, June 2022.

\bibitem{ChPrHo:22}
 Z. Chen, N.P.S Prakash and R. Horowitz,
 \newblock Adaptive Feedforward Reference Design for Active Vibration Rejection in Multi-Actuator Hard Disk Drives 
 \newblock \emph{American Controls Conference}, June 2022.

\bibitem{Mo:19}
Mosek Aps,
\newblock The MOSEK optimization toolbox for MATLAB manual. Version 9.0,
2019, \emph{http://docs.mosek.com/9.0/toolbox/index.html}

\bibitem{Lo:04}
J. Lofberg.
\newblock Yalmip: A toolbox for modeling and optimization
in matlab.
\newblock \emph{IEEE International Symposium on Computer Aided Control Systems
Design}, pages 284--289, 1954.


\bibitem{PrChHo:21}
N.P.S Prakash, Z. Chen and R. Horowitz.
\newblock System Identification in Multi-Actuator Hard Disk Drives with Colored Noises using Observer/Kalman Filter Identification (OKID) Framework, \emph{ArXiv}, volume 2109.12460, 2021.

\bibitem{c7} Simon Haykin and Bernard Widrow, "Least-mean-square adaptive filters", Vol. 31. John Wiley \& Sons, 2003.
%\bibitem{c8} Simon S Haykin, "Adaptive filter theory", Pearson Education India, 2008.
\bibitem{c9} Roberto Horowitz et al., "Dual-stage servo systems and vibration compensation in
computer hard disk drives", Control Engineering Practice 15.3, 2007, pp. 291-305.
%\bibitem{c10} Xinghui Huang, Ryozo Nagamune and Roberto Horowitz, "A comparison of multirate
robust track-following control synthesis techniques for dual-stage and multisensing
servo systems in hard disk drives", IEEE Transactions on magnetics 42.7, 2006,
pp. 1896-1904.
\bibitem{c11} Masahito Kobayashi and Roberto Horowitz, "Track seek control for hard disk dual stage servo systems", IEEE transactions on magnetics 37.2, 2001, pp. 949-954.
%\bibitem{c12} Yunfeng Li and Roberto Horowitz, "Mechatronics of electrostatic microactuators for
computer disk drive dual-stage servo systems", IEEE/ASME transactions on mechatronics 6.2, 2001, pp. 111-121.
\bibitem{c13} Lennart Ljung, "Analysis of recursive stochastic algorithms", IEEE transactions
on automatic control 22.4, 1977, pp. 551-575.
%\bibitem{c14} S Shankar Narayan and AM Peterson, "Frequency domain least-mean-square algorithm", Proceedings of the IEEE 69.1, 1981, pp. 124-126.
\bibitem{c15} F Roosta-Khorasani and MW Mahoney, "Sub-sampled Newton methods 1: Globally
convergent algorithms ", 2006, arXiv preprint arXiv:1601.04737.
\bibitem{c16} Prateek Shah, "Joint Feedback Feedforward Data Driven Control Design and Input
Shaping Techniques for Multi Actuator Hard Disk Drives", PhD thesis, UC Berkeley, 2020.
\bibitem{c17} Prateek Shah and Roberto Horowitz,"Active Vibration Rejection in Multi Actuator Drives: Data Driven Approach", Dynamic Systems and Control Conference, Vol. 59162, American Society of Mechanical Engineers, 2019, V003T17A002.
\bibitem{c18} Behrooz Shahsavari, Jinwen Pan, and Roberto Horowitz, "Adaptive rejection of periodic
disturbances acting on linear systems with unknown dynamics", IEEE
55th Conference on Decision and Control (CDC), IEEE, 2016, pp. 1243-1248.
\bibitem{c19} Behrooz Shahsavari et al., "Adaptive repetitive control design with online secondary
path modeling and application to bit-patterned media recording", IEEE Transactions on Magnetics 51.4, 2015, pp. 1-8.
\bibitem{c20} Behrooz Shahsavari et al., "Adaptive repetitive control using a modified filltered-x lms
algorithm", Dynamic Systems and Control Conference, Vol. 46186, American Society
of Mechanical Engineers, 2014, V001T13A006.
\bibitem{c21} Masayoshi Tomizuka, "Zero phase error tracking algorithm for digital control", Journal of Dynamic Systems, Measurement, and Control, vol. 109, 1987, pp. 65-68.
\bibitem{c22} Zhi Chen, "Feedforward Learning Control For Multi Actuator Hard Drives and Freeform 3D Printers", PhD Thesis, UC Berkeley, 2021.
%\bibitem{c23} MATLAB. version 9.10.0 (R2016b). Natick, Massachusetts: The MathWorks Inc., 2016.
\bibitem{c24} Nikhil Potu Surya Prakash, Zhi Chen and Roberto Horowitz, "Data-Driven  Strictly  Positive  Real  System  Identification  with  prior System  Knowledge",arxiv   preprint,   2021, http://arxiv.org/abs/2110.05672
\bibitem{c32} Shah P., Chen Z., and Horowitz, R, “Application of MIMO Data Driven Feedback Control Design to Dual Stage Hard Disk Drives” ASME 2020 Conference on Dynamics Systems and Control.
\bibitem{c33}Chen Z., Shah P., and Horowitz, R, “Head-Positioning Control in Triple-Stage-Actuator Hard Disk Drives Using Mixed  Synthesis Methodologies” ASME 2020 Conference on Dynamics Systems and Control.
\bibitem{c34}Shah, P., Horowitz, R., "Active Vibration Rejection in Multi Actuator Drives – Data Driven Approach," ASME 2019 Conference on Dynamics Systems and Control.









%\bibitem[Able(1956)]{Abl:56}
%B.C. Able.
%\newblock Nucleic acid content of microscope.
%\newblock \emph{Nature}, 135:\penalty0 7--9, 1956.

%\bibitem[Able et~al.(1954)Able, Tagg, and Rush]{AbTaRu:54}
%B.C. Able, R.A. Tagg, and M.~Rush.
%\newblock Enzyme-catalyzed cellular transanimations.
%\newblock In A.F. Round, editor, \emph{Advances in Enzymology}, volume~2, pages
%  125--247. Academic Press, New York, 3rd edition, 1954.

%\bibitem[Keohane(1958)]{Keo:58}
%R.~Keohane.
%\newblock \emph{Power and Interdependence: World Politics in Transitions}.
%\newblock Little, Brown \& Co., Boston, 1958.

%\bibitem[Powers(1985)]{Pow:85}
%T.~Powers.
%\newblock Is there a way out?
%\newblock \emph{Harpers}, pages 35--47, June 1985.

%\bibitem[Soukhanov(1992)]{Heritage:92}
%A.~H. Soukhanov, editor.
%\newblock \emph{{The American Heritage. Dictionary of the American Language}}.
%\newblock Houghton Mifflin Company, 1992.

\end{thebibliography}
